Analysis and Optimization of Interference Nulling in Downlink Multi-Antenna HetNets with Offloading

Heterogeneous networks (HetNets) with offloading is considered as an effective way to meet the high data rate demand of future wireless service. However, the offloaded users suffer from strong inter-tier interference, which reduces the benefits of offloading and is one of the main limiting factors of the system performance. In this paper, we investigate the use of an interference nulling (IN) beamforming scheme to improve the system performance by carefully managing the inter-tier interference to the offloaded users in downlink two-tier HetNets with multi-antenna base stations. Utilizing tools from stochastic geometry, we derive a tractable expression for the rate coverage probability of the IN scheme. Then, we optimize the design parameter, i.e., the degrees of freedom that can be used for IN, to maximize the rate coverage probability. Specifically, in the asymptotic scenario where the rate threshold is small, by studying the order behavior of the rate coverage probability, we characterize the optimal design parameter. For the general scenario, we show some properties of the optimal design parameter. Finally, by numerical simulations, we show the IN scheme can outperform both the simple offloading scheme without interference management and the almost blank subframes scheme in 3GPP LTE, especially in large antenna regime.

==> begin_code.tex <==
\newtheorem{theorem}{Theorem}
\newenvironment{theorembox} {\begin{theorem}}{\hfill \interlinepenalty500 $\Box$\end{theorem}}
\newtheorem{lemma}{Lemma}
\newenvironment{lemmabox} {\begin{lemma}}{\hfill \interlinepenalty500 $\Box$\end{lemma}}
\newtheorem{corollary}{Corollary}
\newenvironment{corollarybox} {\begin{corollary}}{\hfill \interlinepenalty500 $\Box$\end{corollary}}
\newtheorem{proposition}{Proposition}
\newenvironment{propositionbox} {\begin{proposition}}{\hfill \interlinepenalty500 $\Box$\end{proposition}}
\newtheorem{conjecture}{Conjecture}
\newenvironment{conjecturebox} {\begin{conjecture}}{\hfill \interlinepenalty500 $\Box$\end{conjecture}}
\newtheorem{sketch}{Sketch of Proof}
\newenvironment{sketchbox} {\begin{sketch}}{\hfill \interlinepenalty500 $\Box$\end{sketch}}

\interdisplaylinepenalty=2500

\newcommand{\onecolumnfigurewidth}{1.00\columnwidth}

\newcommand{\figwidth}{11.5cm}


\renewcommand{\baselinestretch}{1.62}

\setlength{\voffset}{-3.5cm} %
\setlength{\hoffset}{-26mm}%
\setlength{\textheight}{22.7cm} %
\setlength{\textwidth}{6.5in}%
\setlength{\columnsep}{0.8cm} %
\setlength{\topmargin}{1in}%
\setlength{\headheight}{5mm} %
\setlength{\headsep}{5mm}%
\setlength{\oddsidemargin}{1in} %
\setlength{\evensidemargin}{0cm}%
\setlength{\parindent}{3.5mm}%

\jot = 1mm
\abovedisplayskip=2.2mm  %  normally about 2.5mm
\belowdisplayskip=2.2mm%
\abovedisplayshortskip = 2.2mm%
\belowdisplayshortskip = 2.2mm%

\pagestyle{fancyplain}


\newcommand{\dis}{\stackrel{d}{\sim}}
\newcommand{\dia}{\stackrel{a}{\sim}}
\newcommand{\uc}{\underline{c}}
\newcommand{\us}{\underline{s}}
\newcommand{\uz}{\underline{z}}
\newcommand{\ue}{\underline{e}}
\newcommand{\uf}{\underline{f}}
\newcommand{\ug}{\underline{g}}
\newcommand{\uhe}{\underline{\hat{e}}}
\newcommand{\uR}{\underline{R}}
\newcommand{\un}{\underline{n}}


\newcommand{\defeq}{\stackrel{\Delta}{=}}
\newcommand{\Real}{\Re e}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bLam}{\mathbf{\Lambda}}
\newcommand{\bSig}{\mathbf{\Sigma}}
\newcommand{\bOm}{\mathbf{\Omega}}
\newcommand{\bPsi}{\mathbf{\Psi}}
\newcommand{\busm}{\mathbf{u}_{s,{\rm max}}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bch}{\mathbf{\hat{c}}}
\newcommand{\beh}{\mathbf{\hat{e}}}
\newcommand{\ubw}{\mathbf{\underline{w}}}
\newcommand{\ube}{\mathbf{\underline{e}}}
\newcommand{\uba}{\mathbf{\underline{a}}}
\newcommand{\ubs}{\mathbf{\underline{s}}}
\newcommand{\ubz}{\mathbf{\underline{z}}}
\newcommand{\ubu}{\mathbf{\underline{u}}}
\newcommand{\ubc}{\mathbf{\underline{c}}}
\newcommand{\ubf}{\mathbf{\underline{f}}}
\newcommand{\ubg}{\mathbf{\underline{g}}}
\newcommand{\ubch}{\mathbf{\underline{\hat{c}}}}
\newcommand{\ubeh}{\mathbf{\underline{\hat{e}}}}
\newcommand{\bwkl}{{\mathbf{w}_{k,\ell}}}
\newcommand{\ubzero}{\mathbf{\underline{0}}}
\newcommand{\lmx}{\lambda_{\rm max}}
\newcommand{\Zon}{\tilde{C}_\mathcal{K}}
\newcommand{\mvgam}{\tilde{\Gamma}}
\newcommand{\Kpart}{\mathcal{K}}

% ----------

